Bridging Adversarial and Nonstationary Multi-armed Bandit

In the multi-armed bandit framework, there are two formulations that are commonly employed to handle time-varying reward distributions: adversarial bandit and nonstationary bandit. Although their oracles, algorithms, and regret analysis differ significantly, we provide a unified formulation in this paper that smoothly bridges the two as special cases. The formulation uses an oracle that takes the best-fixed arm within time windows. Depending on the window size, it turns into the oracle in hindsight in the adversarial bandit and dynamic oracle in the nonstationary bandit. We provide algorithms that attain the optimal regret with the matching lower bound.

==> style/formality.tex <==
\usepackage{hyperref}       % hyperlinks
\hypersetup{
  colorlinks=true,
  linkcolor=red,
  urlcolor=magenta,
  citecolor=blue
}

\usepackage{amsmath,amssymb,amsfonts}
\usepackage{graphicx,color}
\usepackage{url}
\usepackage{subfiles}
\usepackage{booktabs}
\usepackage{mathtools}
\usepackage{microtype}
\usepackage[english]{babel}
\usepackage{caption}
\captionsetup{
  justification=raggedright,
  singlelinecheck=false
  }
\usepackage[toc,page,title,titletoc]{appendix}


==> style/macros.tex <==
\newcommand{\R}{\mathbb{R}} % Real numbers
\newcommand{\Z}{\mathbb{Z}} % Integer numbers
\newcommand{\N}{\mathbb{N}} % Natural numbers

\newcommand{\pr}{\mathbb{P}} % probability
\newcommand{\E}{\mathbb{E}} % expectation
\newcommand{\pro}[1]{\mathbb{P}({#1})} % probability of
\newcommand{\eo}[1]{\mathbb{E}({#1})} % expectation of

\newcommand{\fl}[1]{\lfloor{#1}\rfloor} % floor of a number
\newcommand{\cl}[1]{\lceil{#1}\rceil} % ceiling of a number
\newcommand{\norm}[2]{\|{#2}\|_{#1}} %Norm
\newcommand{\id}[1]{\mathbf{1}_{\{{#1}\}}} %index function

\newcommand{\rcll}{{\it c\`adl\`ag}} % Right continuous with left limits
\newcommand{\D}{\mathbf{D}} % space of cadlag functions
\newcommand{\dto}{\Rightarrow} % weak convergence
\newcommand{\wto}{\stackrel{w}{\to}} % weak convergence
\newcommand{\moc}[3]{\mathbf w_{#3}({#1}(\cdot),{#2})} % modular of continuity

\newcommand{\nnl}{\nonumber\\}

% for highlighting changes
\usepackage[normalem]{ulem}
\newcommand{\delete}[1]{\textcolor{red}{\sout{#1}}} % delete
\newcommand{\ins}[1]{\textcolor{red}{\v{}{#1}}} % insert
\newcommand{\replace}[2]{\textcolor{red}{\sout{#1}}
  \textcolor{blue}{{#2}}} % replace #1 with #2
\newcommand{\emp}[1]{\textcolor{red}{#1}} % emphasize
\newcommand{\cmt}[2]{\textcolor{blue}{({#1}: {#2})}} % comments
\newcommand{\jiheng}[1]{\textcolor{cyan}{{Jiheng: }{#1}}} % comments by Jiheng
